Can Hallucination Correction Improve Video-Language Alignment?

Large Vision-Language Models often generate hallucinated content that is not grounded in its visual inputs. While prior work focuses on mitigating hallucinations, we instead explore leveraging hallucination correction as a training objective to improve video-language alignment. We introduce HACA, a self-training framework learning to correct hallucinations in descriptions that do not align with the video content. By identifying and correcting inconsistencies, HACA enhances the model's ability to align video and textual representations for spatio-temporal reasoning. Our experimental results show consistent gains in video-caption binding and text-to-video retrieval tasks, demonstrating that hallucination correction-inspired tasks serve as an effective strategy for improving vision and language alignment.

==> figures/fig_task1.tex <==
\begin{subfigure}[b]{0.31\textwidth}
\noindent\fbox{%
    % \parbox{\columnwidth}{%
    \parbox[b][6.6cm][c]{\columnwidth}{
    \textbf{Video:} \\ % {tempo/videos/11705.avi}
    \includegraphics[width=.99\textwidth]{images/task_sample_1.pdf} \\
    % \textbf{Task:} Masking completion \\
    \textbf{Input:} {Please correct this caption to accurately describe the video. \\ $\to$ Caption: the \texttt{[MASK]} raises his hand \texttt{[MASK]} man \texttt{[MASK]} to touch top of head} \\
    \textbf{Output:} {the \underline{man} raises his hand \underline{before} man \underline{starts} to touch top of head}
    % ~\\
    }
}
\caption{Masking correction task}
% \vspace{-0.2cm}
\end{subfigure}

==> figures/fig_task2.tex <==
\begin{subfigure}[b]{0.31\textwidth}
\noindent\fbox{%
    % \parbox{\columnwidth}{%
    \parbox[b][6.6cm][c]{\columnwidth}{
    % \centering
    \textbf{Video:} \\ % {tempo/videos/3721.mov} 
    \includegraphics[width=.99\textwidth]{images/task_sample_2.pdf} \\
    % ~\\
    % \textbf{Task:} Entailment\\
    \textbf{Input:} {Does this caption accurately describe the video? \\ $\to$
    Caption: Tennis player tries again then serves the ball} \\
    \textbf{Output:} {\underline{No}}
    ~\\
    ~\\
    ~\\
    ~\\
    % ~\\
    }%
}
\caption{Entailment task}
\end{subfigure}

==> figures/fig_task3.tex <==
\begin{subfigure}[b]{0.31\textwidth}
\noindent\fbox{%
    % \parbox{\columnwidth}{%
    \parbox[b][6.6cm][c]{\columnwidth}{
    \textbf{Video:} \\ % {tempo/videos/15.avi}
    \includegraphics[width=.99\textwidth]{images/task_sample_3.pdf} \\
    % \textbf{Task:} Entailment with hallucination correction \\
    \textbf{Input:} {Does this caption accurately describe the video?\\
    $\to$ Caption: they walk off on the right before someone enters from frame left} \\
    \textbf{Output:} \underline{No. This caption shall} 
    % {
    % \underline{No. This caption shall be } \\
    \underline{be corrected as: \textit{they walk off on}}\\
    \underline{\textit{the right after someone enters}} \\
    \underline{\textit{from frame left}}
    % }
    }
}
\caption{\method{} task}
\end{subfigure}

==> tables/mvbench.tex <==
\begin{table*}[tp]
\centering
% \setlength\tabcolsep{1pt}
% \resizebox{1.0\textwidth}{!}{
\begin{adjustbox}{width=\textwidth}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{l|ccccc!{\color{gray}\vline}ccc!{\color{gray}\vline}cc!{\color{gray}\vline}c!{\color{gray}\vline}cc!{\color{gray}\vline}cc!{\color{gray}\vline}c!{\color{gray}\vline}c!{\color{gray}\vline}ccc>{\columncolor{gray!10}}c}
% \Xhline{1.0pt}
\toprule
& \multicolumn{5}{c!{\color{gray}\vline}}{\textbf{Action}} & \multicolumn{3}{c!{\color{gray}\vline}}{\textbf{Object}} 
& \multicolumn{2}{c!{\color{gray}\vline}}{\textbf{Position}} & \multicolumn{1}{c!{\color{gray}\vline}}{\textbf{Scene}} 
& \multicolumn{2}{c!{\color{gray}\vline}}{\textbf{Count}} & \multicolumn{2}{c!{\color{gray}\vline}}{\textbf{Attribute}} 
& \multicolumn{1}{c!{\color{gray}\vline}}{\textbf{Pose}} & \multicolumn{1}{c!{\color{gray}\vline}}{\textbf{Char.}} 
& \multicolumn{3}{c}{\textbf{Cognition}} & {\textbf{Avg}} \\
\textbf{Model} & \textbf{AS} & \textbf{AP} & \textbf{AA} & \textbf{FA} & \textbf{UA} & \textbf{OE} & \textbf{OI} & \textbf{OS} & \textbf{MD} & \textbf{AL} & \textbf{ST} & \textbf{AC} & \textbf{MC} & \textbf{MA} & \textbf{SC} & \textbf{FP} & \textbf{CO} & \textbf{EN} & \textbf{ER} & \textbf{CI} & {\textbf{ }} \\
\midrule
Random & 25.0 & 25.0 & 33.3 & 25.0 & 25.0 & 33.3 & 25.0 & 33.3 & 25.0 & 25.0 & 25.0 & 33.3 & 25.0 & 33.3 & 33.3 & 25.0 & 33.3 & 25.0 & 20.0 & 30.9 & {27.3}\\
\midrule
mPLUG-Owl-I~\cite{mplug-owl}   & 25.0 & 20.0 & 44.5 & 27.0 & 23.5 & 36.0 & 24.0 & 34.0 & 23.0 & 24.0 & 34.5 & 34.5 & 22.0 & 31.5 & 40.0 & 24.0 & 37.0 & 25.5 & 21.0 & 37.0 & {29.4}\\
LLaMA-Adapter~\cite{llamaadapter}   & 23.0 & 28.0 & 51.0 & 30.0 & 33.0 & 53.5 & 32.5 & 33.5 & 25.5 & 21.5 & 30.5 & 29.0 & 22.5 & 41.5 & 39.5 & 25.0 & 31.5 & 22.5 & 28.0 & 32.0 & {31.7}\\
BLIP2~\cite{blip2}  & 24.5 & 29.0 & 33.5 & 17.0 & 42.0 & 51.5 & 26.0 & 31.0 & 25.5 & 26.0 & 32.5 & 25.5 & 30.0 & 40.0 & 42.0 & 27.0 & 30.0 & 26.0 & 37.0 & 31.0 & {31.4} \\
Otter-I~\cite{otter}   & 34.5 & 32.0 & 39.5 & 30.5 & 38.5 & 48.5 & 44.0 & 29.5 & 19.0 & 25.5 & 55.0 & 20.0 & 32.5 & 28.5 & 39.0 & 28.0 & 27.0 & 32.0 & 29.0 & 36.5 & {33.5}\\
MiniGPT-4~\cite{minigpt4}  & 16.0 & 18.0 & 26.0 & 21.5 & 16.0 & 29.5 & 25.5 & 13.0 & 11.5 & 12.0 & 9.5 & 32.5 & 15.5 & 8.0 & 34.0 & 26.0 & 29.5 & 19.0 & 9.9 & 3.0 & {18.8} \\
InstructBLIP~\cite{instructblip}  & 20.0 & 16.5 & 46.0 & 24.5 & 46.0 & 51.0 & 26.0 & 37.5 & 22.0 & 23.0 & 46.5 & {42.5} & 26.5 & 40.5 & 32.0 & 25.5 & 30.0 & 25.5 & 30.5 & 38.0 & {32.5} \\
LLaVA~\cite{llava}  & 28.0 & 39.5 & 63.0 & 30.5 & 39.0 & 53.0 & 41.0 & 41.5 & 23.0 & 20.5 & 45.0 & 34.0 & 20.5 & 38.5 & 47.0 & 25.0 & 36.0 & 27.0 & 26.5 & 42.0 & {36.0} \\
\midrule
Otter-V~\cite{otter}  & 23.0 & 23.0 & 27.5 & 27.0 & 29.5 & 53.0 & 28.0 & 33.0 & 24.5 & 23.5 & 27.5 & 26.0 & 28.5 & 18.0 & 38.5 & 22.0 & 22.0 & 23.5 & 19.0 & 19.5 & {26.8} \\
mPLUG-Owl-V~\cite{mplug-owl}  & 22.0 & 28.0 & 34.0 & 29.0 & 29.0 & 40.5 & 27.0 & 31.5 & {27.0} & 23.0 & 29.0 & 31.5 & 27.0 & 40.0 & 44.0 & 24.0 & 31.0 & 26.0 & 20.5 & 29.5 & {29.7} \\
VideoChatGPT~\cite{videochatgpt}  & 23.5 & 26.0 & 62.0 & 22.5 & 26.5 & 54.0 & 28.0 & 40.0 & 23.0 & 20.0 & 31.0 & 30.5 & 25.5 & 39.5 & {48.5} & 29.0 & 33.0 & 29.5 & 26.0 & 35.5 & {32.7} \\
VideoLLaMA~\cite{videollama}  & 27.5 & 25.5 & 51.0 & 29.0 & 39.0 & 48.0 & 40.5 & 38.0 & 22.5 & 22.5 & 43.0 & 34.0 & 22.5 & 32.5 & 45.5 & 32.5 & 40.0 & 30.0 & 21.0 & 37.0 & {34.1} \\
VideoChat~\cite{videochat}  & 33.5 & 26.5 & 56.0 & 33.5 & 40.5 & 53.0 & 40.5 & 30.0 & 25.5 & 27.0 & 48.5 & 35.0 & 20.5 & 42.5 & 46.0 & 26.5 & 41.0 & 23.5 & 23.5 & 36.0 & {35.5} \\
\midrule
{VideoChat2$_\mathbf{text}$}  & 24.5 & 27.0 & 49.5 & 27.0 & 38.0 & 53.0 & 28.0 & 40.0 & 25.5 & 27.0 & 38.5 & 41.5 & 27.5 & 32.5 & 46.5 & 26.5 & 36.0 & 33.0 & 32.0 & 40.0 & {34.7} \\
{VideoChat2}  & {66.0} & 47.5 & {83.5} & {49.5} & 60.0 & {58.0} & {71.5} & {42.5} & 23.0 & 23.0 & {88.5} & 39.0 & {42.0} & {58.5} & 44.0 & {49.0} & 36.5 & {35.0} & 40.5 & {65.5} & {{51.1}} \\
\midrule
% VideoLLaVA & 41.5 & 46.5 & -- & 42.0 & 51.5 & 40.5 & 45.5 & 38.5 & 26.5 & 25.5 & 81.0 & 41.0 & 26.0 & 47.0 & 40.5 & -- & 48.5 & 33.0 & -- & 40.0 & {--} \\
\rowcolor[HTML]{F2F3F4} 
\multicolumn{22}{l}{VQA Format} \\
VideoLLaVA & 41.5 & 38.5 & 52.5 & 39.0 & 50.5 & 40.5 & 48.0 & 38.5 & 26.0 & 26.5 & 82.0 & 41.0 & 27.0 & 47.5 & 40.5 & 28.5 & 48.0 & 33.0 & 38.5 & 40.0 & 41.4 \\
$+$ Mask & 31.5 & 26.5 & 51.5 & 31.5 & 36.0 & 52.5 & 41.0 & 38.5 & 25.5 & 26.0 & 40.5 & 37.5 & 24.5 & 39.0 & 34.0 & 34.0 & 42.5 & 35.0 & 26.0 & 34.0 & 35.4 \\
$+$ Entail & 41.0 & 33.0 & 66.0 & 35.0 & 46.0 & 50.5 & 39.0 & 41.5 & 24.0 & 25.0 & 72.0 & 38.5 & 23.5 & 44.5 & 46.5 & 25.0 & 39.0 & 30.5 & 38.5 & 36.5 & 39.8 \\
$+$ Entail+Mask & 42.0 & 40.0 & 54.0 & 34.5 & 53.0 & 50.0 & 49.5 & 42.5 & 25.5 & 24.5 & 79.0 & 35.5 & 27.5 & 44.5 & 32.5 & 31.0 & 43.5 & 32.0 & 40.5 & 31.5 & 40.6 \\
$+$ Entail-Explain & 40.0 & 35.5 & 53.5 & 37.5 & 54.5 & 56.5 & 47.0 & 38.5 & 26.5 & 28.5 &  86.0 & 42.5 & 26.0 & 50.5 & 39.5 & 31.0 & 42.5 & 33.5 & 42.5 & 38.5 & 40.2 \\
$+$ Entail-Explain+Mask & 49.5 & 39.0 & 48.0 & 38.0 & 60.0 & 50.0 & 47.5 & 42.0 & 27.0 & 26.0 & 85.0 & 44.0 & 25.0 & 47.0 & 41.5 & 31.0 & 43.5 & 35.0 & 49.0 & 39.0 & 43.4 \\
\midrule
VideoChat2 & 63.5 & 47.5 & 83.5 & 49.5 & 60.0 & 58.0 & 71.5 & 42.0 & 23.0 & 22.5 & 88.5 & 40.0 & 42.0 & 58.5 & 44.0 & 49.0 & 37.0 & 35.0 & 38.5 & 65.0 & 50.9 \\
$+$ Entail-Explain+Mask$_1$ & 24.0 & 20.0 & 38.0 & 28.5 & 36.5 & 33.5 & 30.0 & 39.0 & 23.0 & 29.0 & 43.0 & 38.5 & 23.5 & 30.0 & 26.0 & 27.5 & 35.5 & 26.0 & 25.0 & 38.0 & 30.7 \\
$+$ Entail-Explain+Mask$_2$ & 1.5 & 0.0 & 30.0 & 16.0 & 25.0 & 0.0 & 4.5 & 19.5 & 0.5 & 2.5 & 14.0 & 14.5 & 28.0 & 5.0 & 9.5 & 20.0 & 17.5 & 25.5 & 13.0 & 6.0 & 12.6 \\
\rowcolor[HTML]{F2F3F4} 
\multicolumn{22}{l}{Entail Format} \\
VideoLLaVA & 46.5 & 48.5 & 56.5 & 32.5 & 47.5 & 43.5 & 50.0 & 33.0 & 26.5 & 28.5 & 70.5 & 33.5 & 31.5 & 51.5 & 57.5 & 30.0 & 43.5 & 27.0 & 33.0 & 39.5 & 41.5 \\
$+$ Mask & 28.5 & 37.0 & 71.0 & 34.5 & 29.5 & 53.0 & 36.5 & 38.0 & 30.5 & 27.5 & 28.0 & 39.5 & 21.0 & 41.5 & 53.0 & 33.0 & 40.5 & 23.5 & 23.5 & 35.5 & 36.2 \\
$+$ Entail & 41.5 & 36.5 & 36.5 & 34.0 & 39.5 & 52.0 & 39.0 & 36.0 & 19.5 & 39.0 & 64.5 & 33.5 & 22.5 & 45.0 & 44.5 & 29.0 & 31.0 & 32.0 & 28.5 & 34.0 & 36.9 \\
$+$ Entail+Mask & 47.5 & 44.5 & 41.0 & 35.0 & 49.0 & 50.5 & 52.0 & 37.5 & 23.0 & 34.0 & 67.0 & 35.0 & 24.5 & 44.5 & 41.5 & 32.5 & 36.5 & 29.0 & 31.0 & 41.0 & 39.8 \\
$+$ Entail-Explain & 47.5 & 33.0 & 52.5 & 36.5 & 40.5 & 46.5 & 48.5 & 40.5 & 24.0 & 31.0 & 78.5 & 38.0 & 19.5 & 49.0 & 42.0 & 32.5 & 44.5 & 28.0 & 32.0 & 38.0 & 40.1 \\
$+$ Entail-Explain+Mask & 50.0 & 36.0 & 7.0 & 38.0 & 41.0 & 22.5 & 54.0 & 40.5 & 21.0 & 33.0 & 79.5 & 47.5 & 26.5 & 46.5 & 30.0 & 31.0 & 35.5 & 23.5 & 30.0 & 37.5 & 36.5 \\
% \multicolumn{23}{l}{\gray{\textit{GPT-4V take \textbf{16} frames as input, and the resolution is \textbf{512$\times$512}, while others use small resolution of \textbf{224$\times$224}.}}} \\
% GPT-4V~\cite{gpt4v} & 55.5 & \textbf{63.5} & 72.0 & 46.5 & \textbf{73.5} & 18.5 & 59.0 & 29.5 & 12.0 & 40.5 & \textbf{83.5} & \textbf{39.0} & 12.0 & 22.5 & 45.0 & 47.5 & 52.0 & 31.0 & \textbf{59.0} & 11.0 &  {43.5} \\
% \textbf{VideoChat2} & \textbf{75.5} & 58.0 & \textbf{83.5} & \textbf{50.5} & 60.5 & \textbf{87.5} & \textbf{74.5} & \textbf{45.0} & \textbf{47.5} & \textbf{44.0} & 82.5 & 37.0 & \textbf{64.5} & \textbf{87.5} & \textbf{51.0} & \textbf{66.5} & \textbf{47.0} & \textbf{35.0} & 37.0 & \textbf{72.5} &  {\textbf{60.4}} \\
% \Xhline{1.0pt}
\bottomrule
\end{tabular}
\end{adjustbox}
% }
% \vspace{-0.3cm}
\caption{Evaluation results on MVBench.}
\label{tab:mvbench}
% \vspace{-0.3cm}
\end{table*}


  
% \begin{table}[tp]
% \centering
% % \setlength\tabcolsep{1pt}
% % \resizebox{1.0\textwidth}{!}{
% \begin{adjustbox}{width=\columnwidth}
% \begin{tabular}{l|cccccccccc|c}
% % \Xhline{1.0pt}
% \toprule
% \textbf{Model} & \textbf{AS} & \textbf{AP} & \textbf{AA} & \textbf{FA} & \textbf{UA} & \textbf{OE} & \textbf{OI} & \textbf{OS} & \textbf{MD} & \textbf{AL} & \cellcolor{gray!10}{\textbf{Avg}} \\
% \midrule
% Random & 25.0 & 25.0 & 33.3 & 25.0 & 25.0 & 33.3 & 25.0 & 33.3 & 25.0 & 25.0 & \cellcolor{gray!10}{27.5}\\
% \midrule
% mPLUG-Owl-I~\cite{mplug-owl}   & 25.0 & 20.0 & 44.5 & 27.0 & 23.5 & 36.0 & 24.0 & 34.0 & 23.0 & 24.0 & \cellcolor{gray!10}{{28.1}}\\
% LLaMA-Adapter~\cite{llamaadapter}   & 23.0 & 28.0 & 51.0 & 30.0 & 33.0 & 53.5 & 32.5 & 33.5 & 25.5 & 21.5 & \cellcolor{gray!10}{{33.2}}\\
% BLIP2~\cite{blip2}  & 24.5 & 29.0 & 33.5 & 17.0 & 42.0 & 51.5 & 26.0 & 31.0 & 25.5 & 26.0 & \cellcolor{gray!10}{{30.6}}\\
% Otter-I~\cite{otter}   & 34.5 & 32.0 & 39.5 & 30.5 & 38.5 & 48.5 & 44.0 & 29.5 & 19.0 & 25.5 & \cellcolor{gray!10}{{34.2}}\\
% MiniGPT-4~\cite{minigpt4}  & 16.0 & 18.0 & 26.0 & 21.5 & 16.0 & 29.5 & 25.5 & 13.0 & 11.5 & 12.0 & \cellcolor{gray!10}{{18.9}}\\
% InstructBLIP~\cite{instructblip}  & 20.0 & 16.5 & 46.0 & 24.5 & 46.0 & 51.0 & 26.0 & 37.5 & 22.0 & 23.0 & \cellcolor{gray!10}{{31.3}}\\
% LLaVA~\cite{llava}  & 28.0 & 39.5 & 63.0 & 30.5 & 39.0 & 53.0 & 41.0 & 41.5 & 23.0 & 20.5 & \cellcolor{gray!10}{{37.9}}\\
% \midrule
% Otter-V~\cite{otter}  & 23.0 & 23.0 & 27.5 & 27.0 & 29.5 & 53.0 & 28.0 & 33.0 & 24.5 & 23.5 & \cellcolor{gray!10}{{29.2}}\\
% mPLUG-Owl-V~\cite{mplug-owl}  & 22.0 & 28.0 & 34.0 & 29.0 & 29.0 & 40.5 & 27.0 & 31.5 & {27.0} & 23.0 & \cellcolor{gray!10}{{29.1}}\\
% VideoChatGPT~\cite{videochatgpt}  & 23.5 & 26.0 & 62.0 & 22.5 & 26.5 & 54.0 & 28.0 & 40.0 & 23.0 & 20.0 & \cellcolor{gray!10}{{32.6}} \\
% VideoLLaMA~\cite{videollama}  & 27.5 & 25.5 & 51.0 & 29.0 & 39.0 & 48.0 & 40.5 & 38.0 & 22.5 & 22.5 & \cellcolor{gray!10}{{34.4}}\\
% VideoChat~\cite{videochat}  & 33.5 & 26.5 & 56.0 & 33.5 & 40.5 & 53.0 & 40.5 & 30.0 & 25.5 & 27.0 & \cellcolor{gray!10}{{36.6}}\\
% \midrule
% {VideoChat2$_\mathbf{text}$}  & 24.5 & 27.0 & 49.5 & 27.0 & 38.0 & 53.0 & 28.0 & 40.0 & 25.5 & 27.0 & \cellcolor{gray!10}{{33.9}}\\
% {VideoChat2}  & {66.0} & 47.5 & {83.5} & {49.5} & 60.0 & {58.0} & {71.5} & {42.5} & 23.0 & 23.0 & \cellcolor{gray!10}{{52.5}}\\
% \midrule
% VideoLLaVA & 41.5 & 46.5 & -- & 42.0 & 51.5 & 40.5 & 45.5 & 38.5 & 26.5 & 25.5 & \cellcolor{gray!10}{{--}}\\
% % \multicolumn{23}{l}{\gray{\textit{GPT-4V take \textbf{16} frames as input, and the resolution is \textbf{512$\times$512}, while others use small resolution of \textbf{224$\times$224}.}}} \\
% % GPT-4V~\cite{gpt4v} & 55.5 & \textbf{63.5} & 72.0 & 46.5 & \textbf{73.5} & 18.5 & 59.0 & 29.5 & 12.0 & 40.5 & \textbf{83.5} & \textbf{39.0} & 12.0 & 22.5 & 45.0 & 47.5 & 52.0 & 31.0 & \textbf{59.0} & 11.0 &  \cellcolor{gray!10}{43.5} \\
% % \textbf{VideoChat2} & \textbf{75.5} & 58.0 & \textbf{83.5} & \textbf{50.5} & 60.5 & \textbf{87.5} & \textbf{74.5} & \textbf{45.0} & \textbf{47.5} & \textbf{44.0} & 82.5 & 37.0 & \textbf{64.5} & \textbf{87.5} & \textbf{51.0} & \textbf{66.5} & \textbf{47.0} & \textbf{35.0} & 37.0 & \textbf{72.5} &  \cellcolor{gray!10}{\textbf{60.4}} \\
% % \Xhline{1.0pt}
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % }
% % \vspace{-0.3cm}
% \caption{Evaluation results on MVBench (part 1).}
% \label{tab:mvpbench}
% % \vspace{-0.3cm}
% \end{table}

% \begin{table}[tp]
% \centering
% % \setlength\tabcolsep{1pt}
% % \resizebox{1.0\textwidth}{!}{
% \begin{adjustbox}{width=\columnwidth}
% \begin{tabular}{l|cccccccccc|c}
% % \Xhline{1.0pt}
% \toprule
% \textbf{Model} & \textbf{ST} & \textbf{AC} & \textbf{MC} & \textbf{MA} & \textbf{SC} & \textbf{FP} & \textbf{CO} & \textbf{EN} & \textbf{ER} & \textbf{CI} & \cellcolor{gray!10}{\textbf{Avg}} \\
% \midrule
% Random & 25.0 & 33.3 & 25.0 & 33.3 & 33.3 & 25.0 & 33.3 & 25.0 & 20.0 & 30.9 & \cellcolor{gray!10}{28.4}\\
% \midrule
% mPLUG-Owl-I~\cite{mplug-owl}   & 34.5 & 34.5 & 22.0 & 31.5 & 40.0 & 24.0 & 37.0 & 25.5 & 21.0 & 37.0 & \cellcolor{gray!10}{30.7}\\
% LLaMA-Adapter~\cite{llamaadapter}   & 30.5 & 29.0 & 22.5 & 41.5 & 39.5 & 25.0 & 31.5 & 22.5 & 28.0 & 32.0 & \cellcolor{gray!10}{30.2}\\
% BLIP2~\cite{blip2}  & 32.5 & 25.5 & 30.0 & 40.0 & 42.0 & 27.0 & 30.0 & 26.0 & 37.0 & 31.0 & \cellcolor{gray!10}{32.1} \\
% Otter-I~\cite{otter}   & 55.0 & 20.0 & 32.5 & 28.5 & 39.0 & 28.0 & 27.0 & 32.0 & 29.0 & 36.5 & \cellcolor{gray!10}{32.7}\\
% MiniGPT-4~\cite{minigpt4}  & 9.5 & 32.5 & 15.5 & 8.0 & 34.0 & 26.0 & 29.5 & 19.0 & 9.9 & 3.0 & \cellcolor{gray!10}{18.7} \\
% InstructBLIP~\cite{instructblip}  & 46.5 & {42.5} & 26.5 & 40.5 & 32.0 & 25.5 & 30.0 & 25.5 & 30.5 & 38.0 & \cellcolor{gray!10}{33.8} \\
% LLaVA~\cite{llava}  & 45.0 & 34.0 & 20.5 & 38.5 & 47.0 & 25.0 & 36.0 & 27.0 & 26.5 & 42.0 & \cellcolor{gray!10}{34.2} \\
% \midrule
% Otter-V~\cite{otter}  & 27.5 & 26.0 & 28.5 & 18.0 & 38.5 & 22.0 & 22.0 & 23.5 & 19.0 & 19.5 & \cellcolor{gray!10}{24.5} \\
% mPLUG-Owl-V~\cite{mplug-owl}  & 29.0 & 31.5 & 27.0 & 40.0 & 44.0 & 24.0 & 31.0 & 26.0 & 20.5 & 29.5 & \cellcolor{gray!10}{30.3} \\
% VideoChatGPT~\cite{videochatgpt}  & 31.0 & 30.5 & 25.5 & 39.5 & {48.5} & 29.0 & 33.0 & 29.5 & 26.0 & 35.5 & \cellcolor{gray!10}{32.8} \\
% VideoLLaMA~\cite{videollama}  & 43.0 & 34.0 & 22.5 & 32.5 & 45.5 & 32.5 & 40.0 & 30.0 & 21.0 & 37.0 & \cellcolor{gray!10}{33.8} \\
% VideoChat~\cite{videochat}  & 48.5 & 35.0 & 20.5 & 42.5 & 46.0 & 26.5 & 41.0 & 23.5 & 23.5 & 36.0 & \cellcolor{gray!10}{34.3} \\
% \midrule
% {VideoChat2$_\mathbf{text}$}  & 38.5 & 41.5 & 27.5 & 32.5 & 46.5 & 26.5 & 36.0 & 33.0 & 32.0 & 40.0 & \cellcolor{gray!10}{35.4} \\
% {VideoChat2}  & {88.5} & 39.0 & {42.0} & {58.5} & 44.0 & {49.0} & 36.5 & {35.0} & 40.5 & {65.5} & \cellcolor{gray!10}{{49.9}} \\
% \midrule
% VideoLLaVA & 81.0 & 41.0 & 26.0 & 47.0 & 40.5 & -- & 48.5 & 33.0 & -- & 40.0 & \cellcolor{gray!10}{--} \\
% % \multicolumn{23}{l}{\gray{\textit{GPT-4V take \textbf{16} frames as input, and the resolution is \textbf{512$\times$512}, while others use small resolution of \textbf{224$\times$224}.}}} \\
% % GPT-4V~\cite{gpt4v} & 55.5 & \textbf{63.5} & 72.0 & 46.5 & \textbf{73.5} & 18.5 & 59.0 & 29.5 & 12.0 & 40.5 & \textbf{83.5} & \textbf{39.0} & 12.0 & 22.5 & 45.0 & 47.5 & 52.0 & 31.0 & \textbf{59.0} & 11.0 &  \cellcolor{gray!10}{43.5} \\
% % \textbf{VideoChat2} & \textbf{75.5} & 58.0 & \textbf{83.5} & \textbf{50.5} & 60.5 & \textbf{87.5} & \textbf{74.5} & \textbf{45.0} & \textbf{47.5} & \textbf{44.0} & 82.5 & 37.0 & \textbf{64.5} & \textbf{87.5} & \textbf{51.0} & \textbf{66.5} & \textbf{47.0} & \textbf{35.0} & 37.0 & \textbf{72.5} &  \cellcolor{gray!10}{\textbf{60.4}} \\
% % \Xhline{1.0pt}
% \bottomrule
% \end{tabular}
% \end{adjustbox}

% % }
% % \vspace{-0.3cm}
% \caption{Evaluation results on MVBench (part 2).}
% \label{tab:mvpbench}
% % \vspace{-0.3cm}
% \end{table}



==> tables/tvbench.tex <==
\begin{table}[t]
% \vspace{-0.5em}
% \small
\centering
% \setlength{\tabcolsep}{2.5pt}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{lcccccccccc>{\columncolor{gray!10}}c}
\toprule
% & & \multirow{2}{*}{ \cellcolor{white} \textbf{\textbf{MVBench}}} & \multirow{2}{*}{\cellcolor{white} \textbf{\textbf{TVBench}}} & & \multicolumn{9}{c}{\textbf{TVBench}} \\
% \cmidrule{5-14}
\textbf{Model} & \textbf{AC} & \textbf{OC} & \textbf{AS} & \textbf{OS} & \textbf{ST} & \textbf{AL} & \textbf{AA} & \textbf{UA} & \textbf{ES} & \textbf{MD} & \textbf{Avg} \\ 
\hline
Random & 25.0     & 25.0     & 50.0 & 33.3       & 50.0 & 25.0    & 50.0 & 25.0   & 25.0     & 25.0  & 33.3 \\
\midrule
GPT-3.5 Turbo & 27.2     & 18.2     & 44.9 & 32.0       & 53.5 & 26.9    & 45.9 & 29.2   & 26.5     & 26.7  & 33.1  \\
GPT-4o & 28.0     & 21.0     & 48.7 & 33.3       & 53.5 & 25.6    & 50.9 & 25.8   & 28.5     & 22.4   & 33.8 \\
Llama 3 70B & 30.2     & 27.0     & 48.7 & 32.9       & 55.1 & 26.9    & 49.1 & 23.3   & 25.5     & 28.0  & 34.7  \\
\midrule
Idefics3  & 27.1     & 23.0     & 56.8 & 36.9       & 49.2 & 25.6    & 52.2 & 29.2   & 25.5     & 19.8  & 34.5  \\
GPT-4o & 30.8     & 19.6     & 62.1 & 33.3       & 52.4 & 25.0    & 52.5 & 27.5   & 33.0     & 21.6   & 35.8 \\
\midrule
{VideoChat2}$^*$ & 25.9 & 21.6 & 51.7 & 33.3 & 48.1 & 23.1 & 44.7 & 34.2 & 25.0 & 22.8  & 33.0 \\
{ST-LLM } & 25.0     & 35.1     & 49.2 & 36.0       & 54.4 & 31.0    & 45.6 & 32.4   & 24.0     & 20.3   & 35.3 \\
{PLLaVA-7B} & 32.1     & 25.7     & 52.1 & 33.3       & 52.4 & 23.8    & 53.1 & 27.5   & 20.5     & 21.6  & 34.2  \\
{PLLaVA-13B} & 37.3     & 24.3     & 57.6 & 33.3       & 55.1 & 28.1 & 47.8 & 35.0   & 19.5     & 17.2  & 35.5  \\
{PLLaVA-34B} & 27.6     & 32.4     & 64.8 & 35.6       & 77.8 & 44.4    & 58.8 & 31.7   & 27.0     & 19.4   & 41.9 \\
{Tarsier-7B} & 22.9     & 58.8     & 70.1 & 35.6       & 64.9 & 46.9    & 75.6 & 32.5   & 25.5     & 25.0  & 45.8  \\
{Tarsier-34B} & 31.7     & 64.2     & 77.1 & 32.1       & 77.8 & 58.1    & 84.4 & 40.0   & 24.5     & 48.3   & 53.8 \\ 
VideoGPT+ & 30.6     & 52.0     & 60.2 & 36.9       & 69.2 & 40.0    & 53.1 & 28.3   & 16.0     & 28.5  & 41.5  \\
Gemini 1.5 Pro & 33.5     & 22.3     & 70.4 & 34.5       & 82.6 & 51.6    & 77.8 & 33.3   & 25.0     & 33.6   & 46.5 \\
% \midrule
% VideoLLaVA & 17.72 & 29.05 & 50.19 & 34.22 & 61.62 & 27.50 & 50.00 & 40.83 & 27.00 & 27.16 & 36.5 \\ 
% $+$ Entail & 26.49 & 21.62 & 44.51 & 36.00 & 66.49 & 33.12 & 46.25 & 25.00 & 34.50 & 20.69 & 35.5 \\
% $+$ Entail $\to$ Explain + Mask & 29.85 & 22.30 & 53.98 & 41.33 & 72.97 & 29.38 & 54.06 & 27.50 & 33.50 & 25.00 & 39.0 \\
\midrule
% \rowcolor[HTML]{F2F3F4} 
% \multicolumn{12}{l}{VQA Format} \\
% VideoLLaVA & 25.0 & 29.0 & 50.2 & 33.3 & 54.0 & 25.6 & 50.6 & 29.2 & 26.0 & 23.7 & 34.7 \\
% $+$ Mask & 25.0 & 23.6 & 49.0 & 33.8 & 53.5 & 28.1 & 46.9 & 23.3 & 27.5 & 22.8 & 33.3 \\
% $+$ Entail & 25.0 & 23.0 & 54.4 & 31.1 & 62.7 & 24.4 & 50.0 & 26.7 & 25.0 & 20.3 & 34.3 \\
% $+$ Entail+Mask & 27.6 & 23.6 & 47.4 & 37.8 & 52.4 & 25.6 & 43.8 & 23.3 & 25.0 & 21.6 & 32.8 \\
% $+$ Entail-Explain & 25.9 & 23.6 & 56.8 & 33.3 & 54.0 & 27.5 & 50.6 & 25.0 & 24.0 & 24.1 & 34.5 \\
% $+$ Entail-Explain+Mask & 25.9 & 21.6 & 55.3 & 33.8 & 53.0 & 26.9 & 48.4 & 24.2 & 26.0 & 23.7 & 33.9 \\
% \rowcolor[HTML]{F2F3F4} 
% \multicolumn{12}{l}{Entail Format} \\
\arrayrulecolor{gray!50}
\hdashline
\rowcolor[HTML]{F2F3F4} 
VideoLLaVA & 17.7 & 29.0 & 50.2 & 34.2 & 61.6 & 27.5 & 50.0 & 40.8 & 27.0 & 27.2 & 36.5 \\
\hdashline
\arrayrulecolor{black}
% $+$ Mask & 28.4 & 26.3 & 50.4 & 32.0 & 50.3 & 28.1 & 51.9 & 25.0 & 26.0 & 28.9 & 34.7 \\
% $+$ Entail & 26.5 & 21.6 & 44.5 & 36.0 & 66.5 & 33.1 & 46.2 & 25.0 & 34.5 & 20.7 & 35.4 \\
% $+$ Entail+Mask & 30.0 & 22.3 & 49.4 & 36.9 & 66.5 & 26.9 & 50.0 & 25.8 & 30.0 & 21.1 & 35.9 \\
% $+$ Entail-Explain & 32.8 & 16.9 & 53.2 & 40.0 & 67.6 & 26.9 & 53.7 & 30.0 & 28.0 & 25.4 & 37.4 \\
$+$ Entail-Explain+Mask & 29.8 & 22.3 & 54.0 & 41.3 & 73.0 & 29.4 & 54.1 & 27.5 & 33.5 & 25.0 & 39.0 \\
% \midrule
\arrayrulecolor{gray!50}
\hdashline
\rowcolor[HTML]{F2F3F4} 
VideoChat2 & 25.0 & 22.3 & 52.5 & 33.3 & 51.4 & 23.8 & 45.0 & 25.0 & 21.0 & 21.6 & 32.1 \\
\hdashline
\arrayrulecolor{black}
% $+$ Entail-Explain+Mask$_1$ & 23.1 & 21.6 & 52.3 & 32.9 & 51.9 & 21.9 & 47.2 & 25.0 & 25.0 & 24.1 & 32.5 \\
$+$ Entail-Explain+Mask & 22.4 & 20.9 & 55.9 & 33.3 & 61.6 & 24.4 & 49.1 & 29.2 & 28.5 & 23.3 & 34.9 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Accuracy of text-only, image only and Video-LLM models on TVBench. $^*$ indicate numbers reported in \cite{cores2024tvbench}.  }
% \vspace{-2em}
\label{table:tvbench}
\end{table}









